GazeIntent: Adapting dwell-time selection in VR interaction with real-time intent modeling

The use of ML models to predict a user's cognitive state from behavioral data has been studied for various applications which includes predicting the intent to perform selections in VR. We developed a novel technique that uses gaze-based intent models to adapt dwell-time thresholds to aid gaze-only selection. A dataset of users performing selection in arithmetic tasks was used to develop intent prediction models (F1 = 0.94). We developed GazeIntent to adapt selection dwell times based on intent model outputs and conducted an end-user study with returning and new users performing additional tasks with varied selection frequencies. Personalized models for returning users effectively accounted for prior experience and were preferred by 63% of users. Our work provides the field with methods to adapt dwell-based selection to users, account for experience over time, and consider tasks that vary by selection frequency

==> experiments.tex <==
\section{Data Collection Environment}





\subsection{}



  
\subsection{User Study 1}
\subsubsection{Sample Population}
\bdj{Will describe demographics + how sampled, will state that we had an approved IRB from our institution }

\subsubsection{Data Generation} %\textbf{Data Generation: ...}
\bdj{what does data generation mean here? Pre-processing? It seems like this is actually the natural section to go after describing the selection tasks, which lists the data we collect that will be used for modeling (gaze-in-world data, GSR, ...)}
\subsubsection{Data Labelling}


==> method.tex <==




\section{Gaze-based Dwell Model}

\bdj{needs a pre-amble, since this is now the offline modeling section (with it's own results presentation) make that scope clear, describes model methodology/pipeline, training data collection, and model optimization results.}



\subsection{Data Preparation}
Our modeling pipeline takes as input a stream of gaze-in-world (GIW) \bdj{cite? Lappi paper, or Gabe Diaz paper} 3D data that is used to compute the instantaneous velocity, i.e., gaze dynamics. The velocity signal is then pre-processed and used to derive features for training the intent prediction model. 
Thus, our proposed gaze-based model combines two data sources: Continuous data and discrete event-based data.  
\subsubsection{Continuous Feature Generation:} Continuous features are generated directly from the gaze signal. Steps include:\newline
\label{Sec:Pre-Processing}
\textit{Feature Calculation:} First,  we calculate 9 continuous features from successive GIW directions. These include absolute, horizontal, and vertical components of displacement and velocity. 
    
    %\item \textbf{Filtering:} We maintain two types of storage, a raw data array, and an intermediate array\bdj{is this describing the offline or real-time modeling? Likely if offline introduced here then the level of detail on array management can be reduced, it suffices to say that the entire signal from one data recording is pre-processed and features extracted as you currently do in each step.}. The raw data array is larger than the intermediate array and follows a first-in-first-out data management method. First, the live GIW directions are saved in the raw data array. Then, we calculate displacement based on successive GIW directions. To filter noise in the data we apply the Savitsky-Golay (SG)\cite{Holmqvist} to the displacement values. The SG filter performs convolutions over adjacent data points using a low-order polynomial. The number of adjacent points considered (filter size/window) and the order of the polynomial used to fit the data are determined during model development. 


    

\textit{Filtering:} To filter noise in the data we apply the Savitsky-Golay (SG)\cite{Holmqvist} to all the three velocity values. The SG filter performs convolutions over adjacent data points using a low-order polynomial. The number of adjacent points considered (filter size/window) and the order of the polynomial used to fit the data are determined during model development. 

\textit{Outlier Removal}: Velocities over 800\degree /s are considered outliers~\cite{dowiasch2015effects} and are removed from the signal and replaced via linear interpolation. After handling the velocity outliers we calculate absolute, horizontal, and vertical acceleration. 
    


\subsubsection{Discrete Feature Generation:} Discrete event-based features are defined based on fixations and saccades. To calculate these features, we detect fixation and saccades. These events were detected from gaze velocity using the I-VT algorithm~\cite{goldberg}. A fixation was detected when the velocity was below 30\degree/s and the minimum and maximum duration of x msec and y msec respectively; while a saccade was detected when the gaze velocity was over 70\degree/s and minimum and maximum duration of x msec and y msec respectively \asn{confirm this from code} When an event is detected, we keep track of the low-level features~\cite{george2016score}. The event-derived features we included in the model include an Event probability (to indicate the presence or absence of fixation or saccade). Other measures include path length, duration, dispersion, amplitude, and peak velocity during the events. We also calculated statistical measures like M3S2DK (Mean-Median-Mode-Standard Deviation-Skewness-Kurtosis) of gaze velocity during the event. A detailed list of 45 fixation-derived, 44 saccade-derived, and 9 real-time features for each frame, (each frame had 98 features) is described in the Appendix\asn{Add this}. These features are appended to the continuous features in the frame after the event ends. For all other frames, the discrete features have 0s present in the corresponding locations.

%\textbf{Tensor Generation}: Each frame consists of fused continuous and discrete data. We maintain an intermediate array of features for each frame. The number of frames stored in this array is called the timeframe length and is determined during training. 


\subsection{Model Prediction}
The tensor developed in the previous stage is passed to an ML model to determine intent. We trained a 5-Layer long short-term memory (LSTM) model, that consists of 512,256,128, and 64 units of LSTM~\cite{hochreiter1996lstm}. The output of the final layer is passed through to a dense layer with sigmoid activation. The optimal number of frames per window was identified to be 17 and 11 features were selected from a total of 98 features. Detailed procedure for model development is explained in \asn{cite section}. 




\subsection{Data Collection-User Study-1}
We conducted an initial user study to collect data to train the models. The study was approved by the Internal Review Board (IRB) and subjects were paid \$20 for an X hour session. We collected data from 18 subjects (7 females, M age = X). In this study, subjects performed divisibility tests. These tests are used to determine if a given number is divisible by a divisor. 
 We refer to this divisor as the divisibility number (DN).  We considered 4 different DNs ( 2, 5, 9, 11) and explained the rules for these numbers before the start. These numbers were selected based on the difficulty of the tests, with the divisibility tests for 2 and 5 being easier as compared to 9 and 11. Two tasks were designed in VR to collect the data %The first task is the selection task under no cognitive load, the second task is the selection task under cognitive load, and the final task is the recall task.%
The VR environment was developed using Unity and deployed on the Oculus Quest Pro headset with sampling rate of 60Hz. 

\textbf{VR Environment:} Subjects were shown three numbers and asked to perform the test for a given DN. The options were displayed on a 3x3 grid of 9 cubes, with only one row visible at a time. Each cube displayed a randomly generated number. The first, second, and third rows had numbers in the range 0 to 999, 1,000 to 999,999, and 1,000,000 to 999,999,999 respectively. In each row, there was only one number that was divisible by the DN. These numbers and the location of the correct number were determined randomly for each grid. Subjects were asked to select a cube in the grid using an Oculus Pro hand controller. In the VR environment, the floor section was assigned as the reference area. At the start of the study, there were no numbers visible to the subjects. Subjects were asked to point the controller toward the floor and press a button to make a row visible. Subjects then had to identify and select the answer, turning the corresponding cube yellow. Subjects were not able to proceed to the next row until they had selected their answer from the previous row. After selecting their answer, they were asked to again point at the reference section and continue as the previous process. Once the third row was selected, that marked the end of a trial. There were 3 trials in a round, and each round had a distinct DN. % The study concluded 90 minutes after the start or after the completion of three blocks whatever occurred first. These tasks were performed in two scenarios.% 

\subsubsection{Selection Task Under No Cognitive Load}
In this task, subjects performed the tests without additional challenges. This task consisted of two parts. In the first part, one grid was to be solved. Each cube was colored black. In the first part of the task, subjects had to solve the grid. Once they selected three answers they were taken to the second part of the task. In this part, each cube in the grid was assigned a random color. A prompt on the screen informed the users about the answers they had selected previously and asked memorize the color label of cubes corresponding to their answers. Once the participants memorized the colors, they proceeded to the next task.

\subsubsection{Selection Task Under Cognitive Load}
In this task, subjects performed the tests with the additional challenge of remembering the color names. This challenge acted as the induced cognitive load for this task. To increase the likelihood of subjects forgetting colors, we added colors to all the blocks in this stage (though the subjects were not required to memorize the colors). After selecting all three answers on the grid subjects were taken to another different 3x3 grid of numbers that they needed to solve.

\textbf{Recall:} After completion of the second grid of divisibility tests under cognitive load, subjects were asked to speak out the colors they had memorized. These answers were recorded by the experimenter.  

\subsubsection{Data Labeling}
 We needed to identify the instant when subjects decided to select a cube. Thus, the gaze collected only when they were performing the divisibility tests is useful for training the ML model. So, the data collected between a row being made visible and a cube being selected was used for training. We followed the label-assigning rules as described by Alghofaili, et al~\cite{LostInStyle}. The moment of button press to select the cube was considered as trigger. All the frames that existed in a particular interval before the trigger were considered to be ground truth or positive and the rest of the frames were labeled as negative. The positive label interval was determined during model training and selection. 

\subsection{Model Training and Selection}
 We trained and evaluated models to optimize the system configurations and model structure (hyperparameters). System configurations include the optimal number of frames in a window (timeframe length), the size and order of the Savitsky-Golay filter, the label interval, and the stride. 
\begin{figure}[h]
    \centering\includegraphics[width=\textwidth]{ModelSelection.pdf}
    \caption{Model Selection Process \bdj{just put curve PDFs here to highlight them as we cannot see right now, explain the stages in text. }}
    \label{fig:modelselection}
\end{figure}


\subsubsection{Stage-1}
 In the first round of model development, we trained 288 models based on four timeframe lengths [13,15,17,19], SG filter order and size [[1,2], [7, 9,11]], four positive label intervals [0.5,0.75, 1,1.25], and three values of stride [0,1,2].  We used 98 variables for each frame that consisted of 9 continuous, 43 features identified from saccades, 44 features identified from fixations, and 2 Boolean variables indicating the occurrence of fixation and saccade. Data was split temporally, with the first 60 percent of the data for each user being in the training set, the next 15 percent in the validation, and the final 15 percent data being in the test set. After this stage, we identified the top 50 models based on the F1 score.

 \subsubsection{Stage-2}
 In this stage, we started with the 50 best models from stage 1 and trained the model from scratch using the walk-forward training method\asn{Find this paper}. We split the training data from the first stage into five equal blocks temporally. In the first round of training, we trained the model on the first two blocks and validated it on the third block. In the second round, we trained on the first three blocks and validated on the fourth, while in the third round, we trained on the first four blocks and validated on the fifth block. In the final round of training, we trained the model using the entire training data and validated it on the validation set used in the previous stage. After this stage, we identified the top 10 models based on the F1 score. 

\asn{BMDJ: Do you think I need to move shapley result secion before this stage? That would address all of your concerns}
\subsubsection{Stage-3}
As mentioned in the previous section \asn{cite your previous} it is not an efficient approach to use all the features especially when the model is deployed in a real-time environment. To identify important features, we first trained models using all the features and then used Shapley values to identify the most important features. As indicated in table-\asn{reference Shapley table}Continuous variables were most impacting the predictions, followed by fixation Boolean, with these variables appearing in the top 30 most impactful features for all the top 54 models trained in the first stage.  Based on these results we created 3 types of feature sets
 \begin{itemize}
     \item Set-1: Only continuous features
     \item Set-2: Continuous + Boolean indicating the presence and absence of the event
     \item Set-3: The Top-30 most impactful features from SHAP. 
 \end{itemize}

We then compared the performance of the top 10 models for the three feature sets and also a complete set of features. Detailed results are indicated in the results section. After this stage, we found that the model trained on window size 17, SG filter size 11 (order 1), label interval of 1 sec and stride of 2 trained on feature set-2 (9 Continous Features + 2 Event Boolean Features) generated the best results.\asn{refer future table}

\subsection{Model Performance under load}
We induced cognitive load using two factors, color memorization and arithmetic complexity. Color memorization required participants to remember colors while performing division tasks, while arithmetic complexity was introduced using difficult divisibility tests of 9 and 11. We generated 4 sub-datasets (data segments), for Load and No-Load conditions for each of these two factors. We trained the top 10 models identified from model development for all three feature sets, so a total of 30 models were trained for each condition, and each model was trained on the four subsets. A total of 120 models were trained in this stage. We compared these models to the models trained on the complete datasets.


\subsection{Model Verification-User Study-2}
We conducted a second user study to validate the performance of our model. The study was approved by the IRB and subjects were paid \$20 USD for subjects. We recruited 17 subjects (10M, 6F, 1NB), 8 of these subjects were returning from the first user study and 8 were new subjects. As will be indicated in results\asn{Cite results}, we did not find conclusive 
evidence for the impact of memory on model performance, so in the second study, we did not ask users to memorize colors. The tasks and the methods were all deployed on Oculus Quest Pro and were developed in Unity. 

\subsubsection{User Study-2}
We designed the following four tasks:
\begin{itemize}
    \item \textbf{Circle Selection Task:} Participants were asked to select a circle of random size, appearing at a random location. They were asked to select as many circles as possible in 60 seconds.
    \item \textbf{Arithmetic task, same stimulus:} Performing the grid divisibility tests for numbers from session 1 (2,5,9,11)
    \item \textbf{Arithmetic task, different stimulus:} Performing the grid divisibility tests for different numbers (3,4,8,12)
    \item \textbf{Sliding Puzzle Task:} Solving the sliding 9-tile puzzle. In this puzzle, participants needed to rearrange numbers from 1-8 in increasing order from top to bottom by moving them around using an empty block
\end{itemize}

There were four gaze only object selection methods we tested these tasks with,
\begin{itemize}
    \item Static Dwell Time - For selecting an object, Dwell time needs to surpass a static value.
    \item Intent Gating(IG): We did not have access to some of the variables used by Isomoto et al\cite{GazeIntent}, so instead of deploying their exact model we deployed a model based on the framework laid out by them. We waited for dwell on a particular object to surpass a static value and then used our Intent model to predict intent. If the prediction was positive then the corresponding object was selected. 
    \item GazeIntent General Model: Implement our Dwell model that is trained on the data from all the users
    \item GazeIntent Personalized Model: Implement a model that is trained on a subset (60\%) of all users and finetuned on a particular user's data
\end{itemize}

We conducted a pilot study to identify static dwell time for each of the tasks. Based on their responses, we also identified values of constants, T1, T2, T3, and T4 during the pilot. Static Dwell identified for the circle selection, division, and sliding puzzle was 0.3 sec, 1.5 sec, and 1.2 sec respectively.

